Black-Box Uniform Stability for Non-Euclidean Empirical Risk Minimization

We study first-order algorithms that are uniformly stable for empirical risk minimization (ERM) problems that are convex and smooth with respect to $p$-norms, $p \geq 1$. We propose a black-box reduction method that, by employing properties of uniformly convex regularizers, turns an optimization algorithm for H\"older smooth convex losses into a uniformly stable learning algorithm with optimal statistical risk bounds on the excess risk, up to a constant factor depending on $p$. Achieving a black-box reduction for uniform stability was posed as an open question by (Attia and Koren, 2022), which had solved the Euclidean case $p=2$. We explore applications that leverage non-Euclidean geometry in addressing binary classification problems.

==> definitions.tex <==
%! TEX root = main.tex

\usepackage{xparse}
\usepackage{xargs}

\makeatletter % for the arxiv, otherwise the raise link doesn't always work well
\def\Hy@raisedlink@left#1{%
    \ifvmode
        #1%
    \else
        \Hy@SaveSpaceFactor
        \llap{\smash{% \llap{ added
        \begingroup
            \let\HyperRaiseLinkLength\@tempdima
            \setlength\HyperRaiseLinkLength\HyperRaiseLinkDefault
            \HyperRaiseLinkHook
        \expandafter\endgroup
        \expandafter\raise\the\HyperRaiseLinkLength\hbox{%
            \Hy@RestoreSpaceFactor
            #1%
            \Hy@SaveSpaceFactor
        }%
        }}% } to close \llap
        \Hy@RestoreSpaceFactor
        \penalty\@M\hskip\z@ 
    \fi
}
\makeatother

\newcommand\newlink[2]{{\protect\hyperlink{#1}{\normalcolor #2}}}
\makeatletter
\newcommand\newtarget[2]{\Hy@raisedlink@left{\hypertarget{#1}{}}#2} % sometimes better than raisedlink
%\newcommand\newtarget[2]{\Hy@raisedlink{\hypertarget{#1}{}}#2}
\makeatother

% This can be done to reference sections or algorithms or other things
% \hyperref[alg:accelerated_gconvex]{\color{black}\operatorname{RiemaconSC}}

\newcommand\linktoproof[1]{{\normalfont[{\hyperlink{proof:#1}{$\downarrow$}}]}}
%\newcommand\linkofproof[1]{\newtarget{proof:#1}}
\newcommand\linkofproof[1]{\textbf{of \cref{#1}. }\newtarget{proof:#1}}

%=====
\usepackage[bb=boondox]{mathalpha} % doublestruck 0 and 1 and other changes to make mathbb more pretty
%\newcommand{\ones}{\mathds{1}} 
\newcommand{\zeros}{\mathbb{0}} 

%=====
\usepackage{tikz}			
% Usage: \circled{1}[\leq]
\newcommand*\circledaux[1]{\tikz[baseline=(char.base)]{
    \node[shape=circle,draw,inner sep=0.8pt] (char) {#1};}}

\NewDocumentCommand{\circled}{m o }{%
    \IfNoValueTF{#2}{\circledaux{#1}}{\stackrel{\circledaux{#1}}{#2}}%
}
%=====


\newcommand\Hess{\operatorname{Hess}}

\renewcommand\set[1]{\{ #1 \}} % commented out due to a conflict with aistats template
\newcommand\setl[1]{\left\{ #1 \right\}}
\newcommand\setsuch[2]{\{ #1 \mid #2  \}}
\newcommand\setsuchl[2]{\left\{ #1 \mid #2  \right\}}

\newcommand\trans{\top}

\newcommand{\EG}{\newlink{def:acronym_extra_gradient}{EG}}
\newcommand{\ERM}{\newlink{def:acronym_empirical_risk_minimization}{ERM}}
\newcommand{\OGDA}{\newlink{def:acronym_optimistic_gradient_descent_ascent}{ODA}}


\newcommand{\bigo}[1]{O( #1 )}
\newcommand{\bigol}[1]{O\left( #1 \right)}
\newcommand{\bigotilde}[1]{\newlink{def:big_o_tilde}{\widetilde{O}}( #1 )}
\newcommand{\bigotildel}[1]{\newlink{def:big_o_tilde}{\widetilde{O}}\left( #1 \right)}
\newcommand{\bigomega}[1]{\newlink{def:big_o_tilde}{\widetilde{\Omega}}( #1 )}
\newcommand{\bigomegatilde}[1]{\newlink{def:big_o_tilde}{\widetilde{\Omega}}( #1 )}
\newcommandx{\bigop}[2][1=,2=p, usedefault]{O_{#2}( #1 )}
\newcommandx{\bigopl}[2][1=,2=p, usedefault]{O_{#2}\left( #1 \right)}
\newcommand{\bigotildepl}[2]{\widetilde{O}_{#1}\left( #2 \right)}
\newcommand{\bigotildep}[2]{\widetilde{O}_{#1}( #2 )}

\newcommand{\return}{\textbf{return}}

\newcommandx*{\reg}[2][1=T, 2=, usedefault]{\operatorname{Reg}_{#1}^{#2}}
\newcommandx*{\regs}[1][1=d, usedefault]{\reg[#1][s]}
\newcommandx*{\regw}[1][1=d, usedefault]{\reg[#1][w]}


\newcommand\conv[1]{\newlink{def:conv}{\operatorname{conv}}\{#1\}}

\renewcommand\dim{d} 
\newcommand\Rd{\R^{\dim}} 

%========
\usepackage{cancel}
% Allows to change the color of the \cancel command
\newcommand\Ccancel[2][black]{
    \let\OldcancelColor\CancelColor
    \renewcommand\CancelColor{\color{#1}}
    \cancel{#2}
    \renewcommand\CancelColor{\OldcancelColor}
}

\newcommand\Cbcancel[2][black]{
    \let\OldcancelColor\CancelColor
    \renewcommand\CancelColor{\color{#1}}
    \bcancel{#2}
    \renewcommand\CancelColor{\OldcancelColor}
}
%========

\newcommandx\ballp[3][1=x, 2=R, 3=p, usedefault]{\newlink{def:ball}{\mathcal{B}_{\norm{\cdot}_{#3}}(#1, #2)}}
\newcommandx\ballpzero[2][1=R, 2=p, usedefault]{\newlink{def:ball}{\mathcal{B}_{\norm{\cdot}_{#2}}(#1)}}
\newcommand\stability{\newlink{def:stability}{\mathcal{E}_{\mathrm{stab}}}}
\newcommand\X{\newlink{def:optimization_domain}{\mathcal{X}}}

